Dual Seminorms, Ergodic Coefficients and Semicontraction Theory

Dynamical systems that are contracting on a subspace are said to be semicontracting. Semicontraction theory is a useful tool in the study of consensus algorithms and dynamical flow systems such as Markov chains. To develop a comprehensive theory of semicontracting systems, we investigate seminorms on vector spaces and define two canonical notions: projection and distance semi-norms. We show that the well-known lp ergodic coefficients are induced matrix seminorms and play a central role in stability problems. In particular, we formulate a duality theorem that explains why the Markov-Dobrushin coefficient is the rate of contraction for both averaging and conservation flows in discrete time. Moreover, we obtain parallel results for induced matrix log seminorms. Finally, we propose comprehensive theorems for strong semicontractivity of linear and non-linear time-varying dynamical systems with invariance and conservation properties both in discrete and continuous time.

==> nomenclature.tex <==



\def\qed {{% set up
		\parfillskip=0pt % so \par doesnt push \square to left
		\widowpenalty=10000 % so we dont break the page before \square
		\displaywidowpenalty=10000 % ditto
		\finalhyphendemerits=0 % TeXbook exercise 14.32
		%
		% horizontal
		\leavevmode % \nobreak means lines not pages
		\unskip % remove previous space or glue
		\nobreak % don't break lines
		\hfil % ragged right if we spill over
		\penalty50 % discouragement to do so
		\hskip.2em % ensure some space
		\null % anchor following \hfill
		\hfill % push \square to right
		$\blacksquare$% % the end-of-proof mark
		%
		% vertical
		\par}}
	
	
\newenvironment{mypro}[1][\hspace{2.3mm} Proof]{\begin{trivlist} 
		\item[\hskip \labelsep {\itshape #1:}]}{\qed \end{trivlist} }

%\newtheorem{mypro}{Proof}
%\renewcommand{\mypro}{\normalfont}
\newtheorem{mythe}{Theorem}
\newtheorem{myrem}[mythe]{Remark}
%\renewcommand{\myrem}{\normalfont}
\newtheorem{myexp}[mythe]{Example}
\newtheorem{mylem}[mythe]{Lemma}
\newtheorem{mydef}[mythe]{Definition}
\newtheorem{myprop}[mythe]{Proposition}
\newtheorem{mycor}[mythe]{Corollary}
\newtheorem{myconj}[mythe]{Conjecture}
%\theoremstyle{definition}


\newcommand{\bma}[2]       {\left[\begin{array}{#1}#2\end{array}\right]}	
\newcommand{\mrm}[1]       {\mathrm{#1}}
\newcommand{\vertcat}[3]   {\mrm{col}_{#2}^{#3} \left( #1 \right)}



\newcommand{\topo}[0]{T}
\newcommand{\topoest}[0]{T^{\Psi}}
\newcommand{\comm}[1]{\mathbb{#1}}
\newcommand{\commstack}[1]{\underline{\mathbb{#1}}}
\newcommand{\commaug}[1]{\underline{\hat{#1}}}
\newcommand{\commaugstack}[1]{{\underline{{#1}}}}
\newcommand{\sel}[2]{{S}_{#1 #2}}
\newcommand{\colstate}[1]{\underline{#1}}
\newcommand{\kron}{\raisebox{1pt}{\ensuremath{\:\otimes\:}}} 
\newcommand{\colspace}[1]     {\mathcal{R}\left(#1\right)}   % The image space
\newcommand{\diag}[1]      {\mrm{{\diagonal}}\!\left(#1\right)}	
\newcommand{\diagIndtwo}[3]      {\mrm{\diagonal}_{#1}^{#2}\!\left(#3\right)}		
\newcommand{\concatIndtwo}[3]      {\mrm{concat}_{#1}^{#2}\!\left(#3\right)}		
\newcommand{\trans}        {\top}																				  % Transposed
\newcommand{\Is}{\underline{I}}


\newcommand{\kronecker}[2] {{#1}\otimes{#2}}
\newcommand{\pat} {P}
\newcommand{\decent}[1] {{#1}^d}
\newcommand{\inter}[1] {{#1}^i}

\newcommand{\Plant}[0]{G}
\newcommand{\Plantclp}[0]{\mathcal{G}}
\newcommand{\plant}[1]{{#1}^{G}}
\newcommand{\clp}[1]{{#1}^{c}}

\newcommand{\cont}[1]{{#1}^{K}}
\newcommand{\contmirror}[1]{{#1}^{KM}}
\newcommand{\plantmirror}[1]{{#1}^{GM}}

\newcommand{\xK}[0]{x^K}
\newcommand{\xP}[0]{x}
\newcommand{\xc}[0]{x^{c}}
\newcommand{\dotxK}[0]{\dot{x}^K}
\newcommand{\dotxP}[0]{\dot{x}}
\newcommand{\dotxc}[0]{\dot{x}^{c}}
\newcommand{\AK}[0]{A^K}
\newcommand{\BK}[0]{B^K}
\newcommand{\CK}[0]{C^K}
\newcommand{\DK}[0]{D^K}

\newcommand{\bd}[1]   {{#1}^d}
\newcommand{\obd}[1]   {{#1}^i}

\newcommand{\gammainv}[0]{\nu} %performance output
\newcommand{\aalpha}[0]   {\alpha}
\newcommand{\intercN}[0]  {\beta}

\newcommand{\perfo}[0]{{z}} %performance output
\newcommand{\perfi}[0]{{w}} %performance input
\newcommand{\intercPo}[0]{q} %performance output
\newcommand{\intercPi}[0]{p} %performance output
\newcommand{\intercKo}[0]{q^K} %performance output
\newcommand{\intercKi}[0]{p^K} %performance output
\newcommand{\interco}[0]{q^c} %performance output
\newcommand{\interci}[0]{p^c} %performance output

\newcommand{\X}[0]{V} %performance output
\newcommand{\Xdag}[0]{U} %performance output

%\newcommand{\seminorm}[0]{\lvert\!\lvert\!\lvert}

